Creativity Inspired Zero-Shot Learning

Zero-shot learning (ZSL) aims at understanding unseen categories with no training examples from class-level descriptions. To improve the discriminative power of zero-shot learning, we model the visual learning process of unseen categories with inspiration from the psychology of human creativity for producing novel art. We relate ZSL to human creativity by observing that zero-shot learning is about recognizing the unseen and creativity is about creating a likable unseen. We introduce a learning signal inspired by creativity literature that explores the unseen space with hallucinated class-descriptions and encourages careful deviation of their visual feature generations from seen classes while allowing knowledge transfer from seen to unseen classes. Empirically, we show consistent improvement over the state of the art of several percents on the largest available benchmarks on the challenging task or generalized ZSL from a noisy text that we focus on, using the CUB and NABirds datasets. We also show the advantage of our approach on Attribute-based ZSL on three additional datasets (AwA2, aPY, and SUN). Code is available.

==> rebuttal.tex <==
{We thank all reviewers for their constructive comments.  We are encouraged that the reviewers find our work as  {{interesting and new (R 1,3,4)}}, {{easy-to-read with well explained ideas and abundant experiments (R1,3)}} }.
                                  
\begin{figure}[ht!]
	\centering
	\vspace{-3mm}
 \includegraphics[width=0.38\textwidth]{ParakeetAuklet_vs_CrestedAukletAUC.png}
	\caption{Seen Unseen Curve for Parakeet Auklet (Seen) on the y-axis versus Crested Auklet (unseen) on the x-axis for GAZSL[57]    GAZSL[57]+our CIZSL loss.}
		\vspace{-3mm}
	\label{fig_auklet}
\end{figure}

% We will move this experiment to the main paper.  

\noindent \textbf{R3,R4 (Analysis):}
Our contribution is orthogonal to existing generative zero-shot learning models (e.g., GAZSL[57] and  FeatGen[53] and cycle-(U)WGAN [B]) since it is a learning signal that improves their performance and can be easily integrated to any of them (see  Sec4.2 in the paper). Fig~\ref{fig_auklet} illustrates the key advantage of our added loss,  doubling the capability of [57] from 0.13 AUC to 0.27 AUC  to distinguish between two very similar birds: Parakeet Auklet (Seen class) and Crested Auklet (unseen class), in 200-way classification. {The text description of both Auklets are similar and the key difference is the Crested Auklet is featured with forehead crests,  made of black forward-curving feathers. }We will add this analysis to the discussion in the main paper. {Detailed explanation of this experiment and bigger version of the figure is attached in supp.} We performed this analysis and t-SNE visualization of the embeddings (Sec6 in supp) as it relates to the learning capability we model. %\elfeki{this is not necessary?}.
%We will consider adding more analysis with toy examples in a journal extension of the paper. 



\noindent \textbf{R4: The underlying hypothesis? }  
A key problem in generalized ZSL approaches is the similarity between a seen and an unseen class (e.g., Parakeet vs Crested Auklets). Hence, we encourage discriminative unseen class generations by hallucinating unseen class descriptions ($t^h$) in the neighborhood of seen classes. We tried different ways to hallucinate unseen text $t^h$ but found that simply linear combining two randomly seen classes with a random $\alpha\in[0.2-0.8]$ to be effective (Eq4){in increasing discrimination between seen classes and similar unseen},  see ablations in Table1 in supp. Our formulation models this capability by maximzing the entropy over seen classes  given the  visual generations of the hallucinated similar unseen text $G(t^h, z)$. %Our loss encourages identifying unseen classes by enforcing a high entropy on the seen of their visual feature generations  during training.

% . What encourages the model capability to generalize better on unseen classes is that the visual feature generations ( ) are optimized to be hard to classify to seen classes (high  entropy) including the very similar Parakeet Auklet class. 

%A main reason that makes an unseen class like Crested Auklet challenging to recognize in a generalized ZSL apart is its similarity to the seen Parakeet Auklet class. %seen class descriptions like Crested Auklet are not available during training. 
% We can not use Crested Auklet description during training since it is not accessible.
%Based on the observation, we encourages discriminative unseen class generations by explicitly exploring hard negative space of seen class descriptions; likely to be in the neighborhood of seen classes. 




\noindent  \textbf{R4 (connection to [43,9]:} In addition to the inspiration that we draw from creativity literature [43,9], we note [43,9] do not connect different modalities (text/attributes to vision) and hence we need to design how to explicitly explore the semantic space of class description to benefit recognizing unseen visual classes; L405-422 in the paper.



%   produced from the nated text are encouraged to be hard to classify to seen classes by maximizing the entropy of seen classes. This explicitly encourage the model to be more capable of distinguishing  unseen classes that are similar to seen classes (harder cases).


% Although unseen class descriptions like Crested auklet are not accessible during training in our setting, we can 

% not only the lack of its accessibility of its description during training but  more importantly



% We relied on the idea that the challenging classes are typically those  



%The key idea of our loss is to explicitly explore the unseen classs description space by hallucinating text that is likely the hard negative space of seen class descriptions; likely to be in the neighborhood of seen classes.

% We then extract a learning signal to help distinguish unseen classes from similar seen classes. 

   


\noindent  \textbf{Results (R3, R4).}  In  Table~\ref{tb:awa2_apy_sun}, we report how integrating our loss improves the performance of GAZSL[57], cycle-(U)WGAN [B] ( provided by R4) and FeatGen[53] in attribute based ZSL on AwA2, aPY, and SUN datasets.  For fair comparison, we used the same neural network architecture and training procedure, described in the paper(L349-376) and Sec3 in supp for all the baseline methods and our work. We also performed the requested \textbf{CUB-T1(Attributes)}  experiment with and without our loss on [57]. 
GAZSL[57]: (Top1 Acc 41.7, Seen-Unseen H 55.8), 
GAZSL[57]+CIZSL: (Top1 Acc 42.2, Seen-Unseen H  57.4). We notice that the performance gain is higher in the generalized ZSL metric (Seen-Unseen H); see Table~\ref{tb:awa2_apy_sun}. The improvement is more significant on the  ZSL from noisy Wikipedia descriptions on both [57] and [53](C). For example, the relative SU-AUC performance is improved by 28.9\% for CUB-Easy and 36.78\% for CUB-Hard;  see the gap between \textcolor{blue}{blue}  (ours) and the \textcolor{red}{red} (baseline) curves in Fig4 in the paper. 

 


 
%Quantitative analysis shows significant improvement on CUB especially on the  Seen-Unseen AUC metric gthat measures confusion between seen and unseen classes (e.g., the seen parakeet auklet versus the unseen crested auklet). Table~\ref{tb:nab_cub} shows 
\noindent \textbf{R4 (A,B,C references ):} In addition to GAZSL[57], we performed experiments on [C] that we already cite as [53] in Table 2 in the paper.  We provide additional experiments in Table~\ref{tb:awa2_apy_sun} on B and C[53]. We will cite and discuss A; we were not able to find its code.
. 

% we 
% we also integrated our loss to C cited in the paper as FeatGen[53]; for accessibility results listed here as well. Per R4 request, we integrated our loss to B. 
% We were not able to find an implementation for A but we will cite and discuss it.  





\noindent \textbf{R1:} We appreciate R1`s constructive feedback.  (a) We currently  define the loss in Sec4.1, while section 4.2 shows how it can be simply integrated with existing methods. To add more clarity, we will further structure Sec4.1 into text hallucination and the loss parts.
(b) GAZSL[57] is one of the approaches our loss can be integrated with;  we  briefly cover the relevant details and contrast (L90-95, L231-238,L360-366, L748-784).  
(c) our paper generate images in the feature space (as we mentioned L151-153). This is similar to the baselines that we follow (e.g., [53,57]); our focus is on zero-shot learning not full image generation.
(e) We will fix the typo and “Top part” vs “Bottom part”  for Fig1.


 








\begin{table}[b!]
\hfill
\centering
\vspace{-4mm}
\scalebox{.7}{%
\begin{tabular}{@{}cccccccc@{}}
\toprule
 & \multicolumn{3}{c}{Top-1 Accuracy(\%)} &  & \multicolumn{3}{c}{Seen-Unseen H} \\ \cmidrule(lr){2-4} \cmidrule(l){6-8} 
 & AwA2 & aPY & SUN &  & AwA2 & aPY & SUN \\ \midrule
FeatGen[53] [C] & 54.3 & 42.6 & 60.8 &  & 17.6 & 21.4 & 24.9 \\
FeatGen[53] [C] + \textbf{CIZSL} & 60.1 & 43.8 & 59.4 &  & 19.1 & 24.0 & 26.5 \\
\midrule
cycle-(U)WGAN [B] & 56.2 & 44.6 & 60.3 &  & 19.2 & 23.6 & 24.4 \\
cycle-(U)WGAN [B] + \textbf{CIZSL} & 63.6 & \textbf{45.1} & \textbf{64.2} &  & 23.9 & \textbf{26.2} & 27.6 \\
\midrule
GAZSL[57] & 58.9 & 41.1 & 61.3 &  & 15.4 & 24.0 & 26.7 \\ 
GAZSL[57] + \textbf{CIZSL} & \textbf{67.8} & 42.1 & 63.7 &  & \textbf{24.6} & 25.7 & \textbf{27.8} \\ \bottomrule
\end{tabular}%
}
\caption{Zero-Shot Recognition on class-level attributes of \textbf{AwA2}, \textbf{aPY} and \textbf{SUN} datasets.}
\label{tb:awa2_apy_sun}
\vspace{-1mm}
\end{table}
